Characterizing High-Quality Test Methods: A First Empirical Study

To assess the quality of a test suite, one can rely on mutation testing, which computes whether the overall test cases are adequately exercising the covered lines. However, this high level of granularity may overshadow the quality of individual test methods. In this paper, we propose an empirical study to assess the quality of test methods by relying on mutation testing at the method level. We find no major differences between high-quality and low-quality test methods in terms of size, number of asserts, and modifications. In contrast, high-quality test methods are less affected by critical test smells. Finally, we discuss practical implications for researchers and practitioners.

==> BGtables.tex <==
\begin{table*}[ht]
\centering
\caption{VVVVV}
\label{tab:tab:mutationExplanation1}
\begin{tabular}{ll | lr | cl}
\toprule
Production & \multirow{2}{*}{Test Method} & \multicolumn{2}{c|}{Parameters} & Expected & \multirow{2}{*}{(Mutant $\rightarrow$ Obtained Result)} \\
Method & & x & y & Result & \\
\midrule
\multirow{3}{*}{sum} & testSum1 & 4 & 5 & 9 & ({\color{red} (1)} $\rightarrow$ -1), ({\color{MyPink} (2)} $\rightarrow$ 0) \\
 & testSum2 & 6 & -5 & 1 & ({\color{red} (1)} $\rightarrow$ 11), ({\color{MyPink} (2)} $\rightarrow$ 0) \\
 & testSum3 & 2 & 0 & 2 & ({\color{red} (1)} $\rightarrow$ 2*), ({\color{MyPink} (2)} $\rightarrow$ 0) \\
\midrule
\multirow{3}{*}{min} & testMin1 & 4 & 5 & 4 & ({\color{blue} (3)} $\rightarrow$ 5), ({\color{MyPink} (4)} $\rightarrow$ 0), ({\color{MyPink} (5)} $\rightarrow$ 4*) \\
 & testMin2 & 6 & -5 & -5 & ({\color{blue} (3)} $\rightarrow$ 6), ({\color{MyPink} (4)} $\rightarrow$ -5*), ({\color{MyPink} (5)} $\rightarrow$ 0) \\
 & testMin3 & 2 & 0 & 0 & ({\color{blue} (3)} $\rightarrow$ 2), ({\color{MyPink} (4)} $\rightarrow$ 0*), ({\color{MyPink} (5)} $\rightarrow$ 0*) \\
\midrule
\multirow{3}{*}{square} & testSquare1 & 0 & -- & 0 & ({\color{green} (6)} $\rightarrow$ 0*), ({\color{MyPink} (7)} $\rightarrow$ 0*) \\
 & testSquare2 & -2 & -- & 4 & ({\color{green} (6)} $\rightarrow$ 4*), ({\color{MyPink} (7)} $\rightarrow$ 0) \\
 & testSquare3 & 4 & -- & 16 & ({\color{green} (6)} $\rightarrow$ 16*), ({\color{MyPink} (7)} $\rightarrow$ 0) \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[ht]
\centering
\caption{XXXXX}
\label{tab:mutationExplanation2}
\include{ExampleTable}
\end{table*}

==> Characterizing high quality test methods - Camera-ready/BGtables.tex <==
\begin{table*}[ht]
\centering
\caption{VVVVV}
\label{tab:tab:mutationExplanation1}
\begin{tabular}{ll | lr | cl}
\toprule
Production & \multirow{2}{*}{Test Method} & \multicolumn{2}{c|}{Parameters} & Expected & \multirow{2}{*}{(Mutant $\rightarrow$ Obtained Result)} \\
Method & & x & y & Result & \\
\midrule
\multirow{3}{*}{sum} & testSum1 & 4 & 5 & 9 & ({\color{red} (1)} $\rightarrow$ -1), ({\color{MyPink} (2)} $\rightarrow$ 0) \\
 & testSum2 & 6 & -5 & 1 & ({\color{red} (1)} $\rightarrow$ 11), ({\color{MyPink} (2)} $\rightarrow$ 0) \\
 & testSum3 & 2 & 0 & 2 & ({\color{red} (1)} $\rightarrow$ 2*), ({\color{MyPink} (2)} $\rightarrow$ 0) \\
\midrule
\multirow{3}{*}{min} & testMin1 & 4 & 5 & 4 & ({\color{blue} (3)} $\rightarrow$ 5), ({\color{MyPink} (4)} $\rightarrow$ 0), ({\color{MyPink} (5)} $\rightarrow$ 4*) \\
 & testMin2 & 6 & -5 & -5 & ({\color{blue} (3)} $\rightarrow$ 6), ({\color{MyPink} (4)} $\rightarrow$ -5*), ({\color{MyPink} (5)} $\rightarrow$ 0) \\
 & testMin3 & 2 & 0 & 0 & ({\color{blue} (3)} $\rightarrow$ 2), ({\color{MyPink} (4)} $\rightarrow$ 0*), ({\color{MyPink} (5)} $\rightarrow$ 0*) \\
\midrule
\multirow{3}{*}{square} & testSquare1 & 0 & -- & 0 & ({\color{green} (6)} $\rightarrow$ 0*), ({\color{MyPink} (7)} $\rightarrow$ 0*) \\
 & testSquare2 & -2 & -- & 4 & ({\color{green} (6)} $\rightarrow$ 4*), ({\color{MyPink} (7)} $\rightarrow$ 0) \\
 & testSquare3 & 4 & -- & 16 & ({\color{green} (6)} $\rightarrow$ 16*), ({\color{MyPink} (7)} $\rightarrow$ 0) \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[ht]
\centering
\caption{XXXXX}
\label{tab:mutationExplanation2}
\include{ExampleTable}
\end{table*}

==> Characterizing high quality test methods - Camera-ready/CodeOverlayMagic.tex <==

\makeatletter
\newenvironment{btHighlight}[1][]
{\begingroup\tikzset{bt@Highlight@par/.style={#1}}\begin{lrbox}{\@tempboxa}}
{\end{lrbox}\bt@HL@box[bt@Highlight@par]{\@tempboxa}\endgroup}

\newcommand\btHL[1][]{%
  \begin{btHighlight}[#1]\bgroup\aftergroup\bt@HL@endenv%
}
\def\bt@HL@endenv{%
  \end{btHighlight}%   
  \egroup
}
\newcommand{\bt@HL@box}[2][]{%
  \tikz[#1]{%
    \pgfpathrectangle{\pgfpoint{1pt}{0pt}}{\pgfpoint{\wd #2}{\ht #2}}%
    \pgfusepath{use as bounding box}%
    \node[anchor=base west, fill=orange!30,outer sep=0pt,inner xsep=1pt, inner ysep=0pt, rounded corners=3pt, minimum height=\ht\strutbox+1pt,#1]{\raisebox{1pt}{\strut}\strut\usebox{#2}};
  }%
}
\makeatother

\lstdefinestyle{Java}{
    language={Java},
    basicstyle=\scriptsize, 
    % moredelim=**[is][\btHL]{`}{`},
    moredelim=**[is][{\btHL[fill=green!30,draw=red,dashed,thin]}]{`}{`},                
    captionpos=b,
    % xleftmargin=.08\textwidth, 
    % xrightmargin=-0.08\textwidth, 
}
\newcommand{\allowHyphen}[1]{{\operatorname{\mathit{#1}}}}

==> Characterizing high quality test methods - Camera-ready/header.tex <==
% \usepackage{cite}X
% \usepackage{amsmath,amssymb,amsfonts}X
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{url}
\usepackage{listings,tikz,beramono}
\usepackage{multirow}
\usepackage{textcomp} % For numero sign
\usepackage{enumitem} % For prettier RQ enumeration
\usepackage{float}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\usepackage{xspace}
\newcommand*{\eg}{\emph{e.g.,}\@\xspace}
\newcommand*{\ie}{\emph{i.e.,}\@\xspace}
\newcommand*{\etal}{\emph{et al.}\@\xspace}
\usepackage{booktabs}
\definecolor{dark green}{rgb}{0.0, 0.7, 0.0}
\usepackage{tcolorbox}

\newlength\MAX  \setlength\MAX{8mm}
\newcommand*\Chart[1]{~\rlap{\textcolor{black!20}{\rule{\MAX}{2ex}}}\rule{#1\MAX}{2ex}}

\definecolor{MyPink}{HTML}{FF00FF}

%\usepackage{caption}
%\usepackage{lastpage209} %For last page -- it is rather obsolete ...
%\usepackage[table,x11names,dvipsnames,table]{xcolor}

%\usepackage{booktabs,array,arydshln}
\usepackage[export]{adjustbox}
%\usepackage{caption}
%\usepackage{subcaption}

%\usepackage{siunitx}        % new, for nicer aligning of numbers in table
%\usepackage{etoolbox}  

==> CodeOverlayMagic.tex <==

\makeatletter
\newenvironment{btHighlight}[1][]
{\begingroup\tikzset{bt@Highlight@par/.style={#1}}\begin{lrbox}{\@tempboxa}}
{\end{lrbox}\bt@HL@box[bt@Highlight@par]{\@tempboxa}\endgroup}

\newcommand\btHL[1][]{%
  \begin{btHighlight}[#1]\bgroup\aftergroup\bt@HL@endenv%
}
\def\bt@HL@endenv{%
  \end{btHighlight}%   
  \egroup
}
\newcommand{\bt@HL@box}[2][]{%
  \tikz[#1]{%
    \pgfpathrectangle{\pgfpoint{1pt}{0pt}}{\pgfpoint{\wd #2}{\ht #2}}%
    \pgfusepath{use as bounding box}%
    \node[anchor=base west, fill=orange!30,outer sep=0pt,inner xsep=1pt, inner ysep=0pt, rounded corners=3pt, minimum height=\ht\strutbox+1pt,#1]{\raisebox{1pt}{\strut}\strut\usebox{#2}};
  }%
}
\makeatother

\lstdefinestyle{Java}{
    language={Java},
    basicstyle=\scriptsize, 
    % moredelim=**[is][\btHL]{`}{`},
    moredelim=**[is][{\btHL[fill=green!30,draw=red,dashed,thin]}]{`}{`},                
    captionpos=b,
    % xleftmargin=.08\textwidth, 
    % xrightmargin=-0.08\textwidth, 
}
\newcommand{\allowHyphen}[1]{{\operatorname{\mathit{#1}}}}
